Comment on the claim of physical irrelevance of the topological term

We argue that the claim of the absence of charge-conjugation-parity (CP) violating effects due to a topological term in quantum chromodynamics (QCD) is based upon a misunderstanding, and the standard results in the field are correct.

==> acronyms.tex <==
%% Acronyms
\usepackage{relsize}
% \usepackage[smaller]{acronym}

\usepackage[acronyms, nohypertypes={acronym}, nopostdot, style=super, nonumberlist, toc]{glossaries}
\glsenableentrycount
% \usepackage{glossaries-extra}
% \makenoidxglossaries
%\makeglossaries  
\setacronymstyle{long-sc-short}

% \makeatletter
% \patchcmd{\AC@aclp}{\AC@acl{#1}s}{\AC@acl{#1}{\normalsize s}}{}{}
% \patchcmd{\AC@acsp}{\AC@acs{#1}s}{\AC@acs{#1}{\normalsize s}}{}{}
% \makeatother

\newcommand\acrodef[2]{\newacronym{#1}{#1}{#2}}
\newcommand\ac[1]{\gls{#1}}
\newcommand\acp[1]{\glspl{#1}}
\newcommand\Acp[1]{\glspl{#1}}
\def\acresetall{\glsresetall[acronym]}

% \newacronym{WF}{wf}{Wilson-Fisher}
\newacronym{WF}{wf}{Wilson-Fisher}
\newacronym{AF}{af}{asymptotically free}

\newacronym{RG}{rg}{renormalization group}

\newacronym{QEC}{qec}{quantum error correction}

% \newacronym{LFT}{lft}{lattice field theory}
% \acrodefplural{LFT}{lattice field theories}

\newacronym[longplural={conformal field theories}]{CFT}{cft}{conformal field theory}
\newacronym[longplural={lattice field theories}]{LFT}{lft}{lattice field theory}
\newacronym[longplural={effective field theories}]{EFT}{eft}{effective field theory}
\newacronym[longplural={quantum field theories}]{QFT}{qft}{quantum field theory}

% \newacronym{QFT}{qft}{quantum field theory}
% \acrodefplural{QFT}{quantum field theories}
% \newglossaryentry{QFT}
% {
%   name={qft},
%   description={quantum field theory},
%   descriptionplural={quantum field theories},
% }


\newacronym{JLP}{jlp}{Jordan-Lee-Preskill}

\newacronym{BBN}{bbn}{big bang nucleosynthesis}

\newacronym{LEC}{lec}{low-energy constant}
% \acrodefplural{LEC}{low-energy constants}

\newacronym{QCD}{qcd}{quantum chromodynamics}
\newacronym{MC}{mc}{Monte Carlo}

\newacronym{IR}{ir}{infrared}
\newacronym{UV}{uv}{ultraviolet}

\newacronym{QED}{qed}{quantum electrodynamics}
\newacronym{SNR}{snr}{signal-to-noise ratio}

\newacronym{NLSM}{nlsm}{nonlinear sigma model}

\newacronym{CL}{cl}{Complex Langevin}

\newacronym{CSA}{csa}{Cartan subalgebra}

\newacronym{SSB}{ssb}{spontaneous symmetry breaking}

\newacronym{AFQMC}{afqmc}{auxiliary field quantum Monte Carlo}
\newacronym{iHMC}{ihmc}{imaginary-mass Hybrid Monte Carlo}

\newacronym{MCMC}{mcmc}{Markov Chain Monte Carlo}
\newacronym{WZW}{wzw}{Wess-Zumino-Witten}

